Spatially Adaptive Projective Integration Schemes For Stiff Hyperbolic Balance Laws With Spectral Gaps

Stiff hyperbolic balance laws exhibit large spectral gaps, especially if the relaxation term significantly varies in space. Using examples from rarefied gases and the general form of the underlying balance law model, we perform a detailed spectral analysis of the semi-discrete model that reveals the spectral gaps. Based on that, we show the inefficiency of standard time integration schemes expressed by a severe restriction of the CFL number. We then develop the first spatially adaptive projective integration schemes to overcome the prohibitive time step constraints of standard time integration schemes. The new schemes use different time integration methods in different parts of the computational domain, determined by the spatially varying value of the relaxation time. We use our analytical results to derive accurate stability bounds for the involved parameters and show that the severe time step constraint can be overcome. The new adaptive schemes show good accuracy in a numerical test case and can obtain a large speedup with respect to standard schemes.

==> secLSA.tex <==
\section{Model equations}
We look at systems of the following form
\begin{equation}
\label{e:vars_system1D}
    \frac{\partial \Var_M}{\partial t}  + \Vect{A} \frac{\partial \Var_M}{\partial x}  = \Vect{S}(\Var_M),
\end{equation}
where $\Var_M \in \mathbb{R}^{N}$ is the unknown variable, $\Vect{A} \in \mathbb{R}^{N \times N}$ the system matrix, and $\Vect{S} \in \mathbb{R}^{N}$ the possibly stiff right-hand side.


\subsection{Scalar equation}
The simplest form of the model equation \eqref{e:vars_system1D} considered in this paper is
\begin{equation}
\label{e:scalar}
    \frac{\partial w}{\partial t}  + a \frac{\partial w}{\partial x}  = - \frac{1}{\tau} w,
\end{equation}
which models a transport with constant velocity $a\in \mathbb{R}$ and relaxation to zero with relaxation rate $\frac{1}{\tau}$. Note that the constant transport velocity leads to a time step constraint of the form $\Delta t \leq CFL \frac{1}{a \Delta x}$ for given CFL number $CFL \leq 1$. For small values of $\tau$, the right-hand sides lets the equation becomes stiff and leads to the constraint $\Delta t < \frac{1}{\tau}$.


\subsection{Hyperbolic moment models}
The non-linear hyperbolic moment model (HME) is given by the system matrix
\begin{equation}
\label{e:QBME_A}
\Vect{A}_{HME} = \setlength{\arraycolsep}{1pt}
\left(
  \begin{array}{cccccccc}
    \vel & \rho &  &  &   &   &   &  \\
    \frac{\theta}{\rho} & \vel & 1 &  &  &   &   &  \\
    & 2 \theta & \vel & \frac{6}{\rho} &  &  &   &   \\
    & 4 f_3 & \frac{\rho \theta}{2} & \vel & 4 &  &  &  \\
    -\frac{\theta f_3}{\rho} & 5f_4 & \frac{3f_3}{2} & \theta & \vel & 5 &  &    \\
    %&  &  &  &  &  &  &  & \\
    \vdots & \vdots & \vdots & \vdots &  \ddots & \ddots & \ddots &  \\
    %&  &  &  &  &  &  &  & \\
    -\frac{\theta f_{M-2}}{\rho} & Mf_{M-1} & \frac{\left(M-2\right)f_{M-2}+ \theta f_{M-4}}{2} \textcolor{myred}{-\frac{M(M+1)f_{M}}{2 \theta}}& -\frac{3f_{M-3}}{\rho}  &  & \theta & \vel & M \\
    -\frac{\theta f_{M-1}}{\rho} & (M\hspace{-0.1cm}+\hspace{-0.1cm}1) f_{M} & \textcolor{myred}{-f_{M-1}} \hspace{-0.1cm} + \hspace{-0.1cm} \frac{\theta f_{M-3}}{2} & \textcolor{myred}{\frac{3(M+1)f_{M}}{\rho \theta}} \hspace{-0.1cm} - \hspace{-0.1cm} \frac{3f_{M-2}}{\rho} &  &  & \theta & \vel \\
  \end{array}
\right),
\setlength{\arraycolsep}{6pt}
\end{equation}
and the collision term $\Vect{S}(\Var_M)$ for the simple BGK model is given by
\begin{equation}
\label{e:BGK_term}
    \Vect{S}(\Var_M)  = - \frac{1}{\tau} diag \left( 0,0,0,1, \ldots,1 \right) \Var_M.
\end{equation}
for the following vector of unknown variables
\begin{equation}
    \label{e:vars_full_1D}
    \Var_M = \left( \rho, \vel, \theta, f_3, \ldots, f_M \right)^T.
\end{equation}


\subsection{Hermite spectral model}
The linearized version called Hermite Spectral Method (HSM) is given by the system matrix
\begin{equation}
\label{e:grad_A_HSM}
\Vect{A}_{HSM} = \left(
  \begin{array}{ccccc}
     & 1 &   &   &   \\
     1 &  & \sqrt{2}  &   &   \\
     & \sqrt{2} &   &  \ddots &   \\
     &  & \ddots  &   & \sqrt{M}  \\
     &  &   & \sqrt{M}  &
  \end{array}
\right).
\end{equation}

The right-hand side vector $\vect{S}\left( \Var_M \right) \in \mathbb{R}^{M+1}$ for the 1D BGK model is more complicated and given by
\begin{equation}
  \vect{S}_{\alpha} = \int_{\mathbb{R}} \left( f(t,x,c) - f_M(t,x,c) \right) \psi_{\alpha}(c) \,dc, \quad \textrm{ for } \psi_{\alpha}(c) = He_{\alpha}(c) \cdot \frac{1}{\sqrt{2^{\alpha} {\alpha}!}},
\end{equation}
where an analytical expression is difficult to obtain.


\section{Spatial discretization}
All systems can be discretized in space-time using
\begin{equation}\label{scheme}
    W_i^{n+1}=W_i^n-\frac{\Delta t}{\Delta x}\big(D_{i-1/2}^{+} + D_{i+1/2}^{-}\big),
\end{equation}
with
\begin{equation}
    D_{i+1/2}^{\pm}=\widetilde{\Vect{A}}_\Phi^\pm (W_i,W_{i+1})
\end{equation}
given by a polynomial viscosity ansatz
\begin{equation}
    \widetilde{\Vect{A}}_\Phi^\pm (W_L,W_R) =  \frac{1}{2}\left( \Vect{A}_\Phi \cdot (W_L,W_R) \pm \Vect{Q}_\Phi \cdot (W_L,W_R)\right),  \label{fvm}
\end{equation}
with Roe linearization $\Vect{A}_\Phi = \Vect{A}_\Phi(W_L,W_R)$ given by
\begin{equation}\label{Roe-gen}
    \Vect{A}_\Phi(W_L,W_R)\cdot (W_R-W_L)=\int_0^1 \Vect{A} (\Phi(s;W_L,W_R))\frac{\partial\Phi}{\partial s}(s;W_L,W_R)\,ds.
\end{equation}
and viscosity matrix $\Vect{Q}_\Phi = \Vect{Q}_\Phi(W_L,W_R)$ of the form $\Vect{Q}_\Phi(W_i,W_{i+1}) = P_r^{i+1/2}\left(\Vect{Q}_\Phi\left(W_i,W_{i+1}\right)\right)$, where $P^{i+1/2}_r(x)$ is a polynomial of degree $r$, hence the name polynomial viscosity matrix.

Most standard schemes can be written in the PVM form:
\begin{itemize}
%  \item the Roe scheme (TODO)
  \item the Lax-Friedrich scheme uses $r=0$, $P_0(x)=a_0$ and polynomial coefficient
        \begin{equation}
            a_0= \frac{\Delta x}{\Delta t}.
        \end{equation}
  \item the HLL scheme can be written using $r=1$, $P_1(x)=a_0+a_1 x$ and the polynomial coefficients
        \begin{equation}
            a_0=\frac{\lambda_N^{i+1/2}|\lambda_1^{i+1/2}|-\lambda_1^{i+1/2}|\lambda_N^{i+1/2}|}{\lambda^{i+1/2}_N-\lambda^{i+1/2}_1}, a_1=\frac{|\lambda_N^{i+1/2}| - |\lambda_1^{i+1/2}|}{\lambda^{i+1/2}_N-\lambda^{i+1/2}_1},
        \end{equation}
  \item the FORCE scheme uses $r=2$, $P_2(x)=a_0 + a_2x^2$ and polynomial coefficients
        \begin{equation}
            a_0= \frac{\Delta x}{2 \Delta t}, a_2=\frac{ \Delta t}{2 \Delta x}.
        \end{equation}
\end{itemize}

Note that the standard (exact) Roe scheme uses $\Vect{Q}_\Phi(W_i,W_{i+1}) = \left|\Vect{A}_\Phi(W_L,W_R)\right|$, which is not a polynomial and can only be constructed given the full eigenstructure of the model. The polynomial should be as close as possible to the absolute value function while $P_r^{i+1/2}\left(x\right)\geq \left| x \right|$ is required for stability.\\

In the following, we assume an appropriate linearization of the system, i.e. $\Vect{A} = const$, $\Vect{A}_\Phi(W_L,W_R)= \Vect{A}$, $\Vect{Q}_\Phi(W_i,W_{i+1})= \Vect{Q}$

The system \eqref{scheme} with the PVM method can thus be written as
\begin{equation}\label{PVM-scheme}
    \frac{W_i^{n+1}-W_i^n}{\Delta t} = -\frac{1}{\Delta x} \left( \Vect{A} \cdot \frac{ W_{i+1}^n - W_{i-1}^n}{2} + \Vect{Q} \cdot \frac{ - W_{i+1}^n + 2 W_{i}^n - W_{i-1}^n}{2} \right) - \frac{1}{\epsilon} \Vect{S} W_{i}^n,
\end{equation}
where the terms on the right-hand side are the non-conservative numerical flux, the numerical diffusion, and the (potentially stiff) source term.

Writing this as a semi-discrete system and assuming periodic boundary conditions, the system of equations reads
\begin{equation}\label{semi-scheme}
    \frac{\partial \Vect{W}}{\partial t} = \left( - \frac{1}{2 \Delta x} \left( \Vect{A} \cdot \left(
  \begin{array}{ccccc}
     & 1 &   &   & -1  \\
     -1 &  & 1  &   &   \\
     & -1 &   &  \ddots &   \\
     &  & \ddots  &   & 1  \\
     1 &  &   & -1  &
  \end{array}
\right) + \Vect{Q} \cdot \left(
  \begin{array}{ccccc}
     2 & -1 &   &   & -1  \\
     -1 & 2 & -1  &   &   \\
     & -1 & \ddots  &  \ddots &   \\
     &  & \ddots  & \ddots  & -1  \\
     -1 &  &   & -1  & 2
  \end{array}
\right) \right) - \frac{1}{\epsilon} \Vect{S} \right) \Vect{W},
\end{equation}
with $\Vect{W}= \left( W_1^n, \ldots, W_N^n \right)^T$. Note that the matrices need to be multiplied block wise and the entries of the two matrices are $M+1$ by $M+1$ blocks.

The system \eqref{semi-scheme} can be simplified to
\begin{equation}\label{semi-scheme}
    \frac{\partial \Vect{W}}{\partial t} = \widetilde{\Vect{A}} \Vect{W},
\end{equation}
with blockwise defined matrix
\begin{equation}\label{semi-scheme_matrix}
    \widetilde{\Vect{A}} = \left(
  \begin{array}{ccccc}
     a & b &   &   & c  \\
     c & a & b  &   &   \\
     & c & \ddots  &  \ddots &   \\
     &  & \ddots  & \ddots  & b  \\
     b &  &   & c  & a
  \end{array}
\right),
\end{equation}
that has entries
\begin{eqnarray}
  a &=& -\frac{1}{\Delta x} \Vect{Q} - \frac{1}{\epsilon} \Vect{S}, \\
  b &=& \frac{1}{2\Delta x} \left( \Vect{Q} - \Vect{A} \right), \\
  c &=& \frac{1}{2\Delta x} \left( \Vect{Q} + \Vect{A} \right).
\end{eqnarray}

From the definition of the matrix $\widetilde{\Vect{A}}$ we can see that a large value of the entries in $\Vect{Q}$ makes the matrix more diagonally dominant and leads to a more stable scheme.
The case $\Vect{Q}=0$, which corresponds to discretizing the transport part using simple central finite differences, would lead to an instable scheme.


\subsection{Constant relaxation time}
TODO refer to literature and explain slow cluster from relaxation plus transport cluster.

\subsection{Spatially varying relaxation time}
We now assume that the collision rate changes throughout the domain in space, but not in time. This means we have $\epsilon = \epsilon(x)$. We use
\begin{equation}\label{e:collision_rate_adaptive}
    \epsilon(x) = \left\{
  \begin{array}{cl}
    \epsilon_L & \textrm{if } x < 0, \\
    \epsilon_R & \textrm{if } x \geq 0, \\
  \end{array} \right.
\end{equation}
which gives rise to denoting $\Vect{W} = \left( \begin{array}{c}
    \Vect{W}_L \\
    \Vect{W}_R \\
  \end{array} \right)$ and the following decomposition of the system into two regions:
\begin{equation}\label{decoupled-scheme}
    \frac{\partial}{\partial t} \left( \begin{array}{c}
    \Vect{W}_L \\
    \Vect{W}_R \\
  \end{array} \right) =  \left( \begin{array}{cl}
    \Vect{A}_{LL} & \Vect{A}_{LR} \\
    \Vect{A}_{RL} & \Vect{A}_{RR} \\
  \end{array} \right) \left( \begin{array}{c}
    \Vect{W}_L \\
    \Vect{W}_R \\
  \end{array} \right),
\end{equation}
where $\Vect{W}_L$ and $\Vect{W}_R$ correspond to the values in the left part and right part of the domain, respectively.

In terms of \eqref{semi-scheme_matrix} the respective parts of the system are given as
\begin{equation}\label{semi-scheme_matrix}
    \Vect{A}_{LL} = \left(
  \begin{array}{cccc}
     a_L & b &     &   \\
      c & \ddots  &  \ddots &   \\
      & \ddots  & \ddots  & b  \\
       &   & c  & a_L
  \end{array}
\right), \Vect{A}_{LR} = \left(
  \begin{array}{cccc}
      &  &     & c  \\
      &  &     &   \\
     &  &     &   \\
     b &   &   &
  \end{array}
\right),
\end{equation}

\begin{equation}\label{semi-scheme_matrix}
    \Vect{A}_{RL} = \left(
  \begin{array}{cccc}
      &  &     & c  \\
      &  &     &   \\
     &  &     &   \\
     b &  &     &
  \end{array}
\right), \Vect{A}_{RR} = \left(
  \begin{array}{cccc}
     a_R & b &    &   \\
     c & \ddots  &  \ddots &   \\
      & \ddots  & \ddots  & b  \\
       &   & c  & a_R
  \end{array}
\right),
\end{equation}
with
\begin{eqnarray}
  a_L &=& -\frac{1}{\Delta x} \Vect{Q} - \frac{1}{\epsilon_L} \Vect{S}, \\
  a_R &=& -\frac{1}{\Delta x} \Vect{Q} - \frac{1}{\epsilon_R} \Vect{S}.
\end{eqnarray}
Note that the only difference in the two block matrices on the diagonal is the value of the source term, which uses either $\epsilon_L$ for $\Vect{A}_{LL}$ or $\epsilon_R$ for $\Vect{A}_{RR}$, respectively. The very sparse off-diagonal blocks contain the information of the boundary conditions coupling the left and right part of the domain.


The coupled system can be written as two subsystems
\begin{eqnarray}
    \frac{\partial}{\partial t} \Vect{W}_L &=& \Vect{A}_{LL} \cdot \Vect{W}_L + \Vect{A}_{LR} \cdot \Vect{W}_R \label{decoupled-systemsL}, \\
    \frac{\partial}{\partial t} \Vect{W}_R &=& \Vect{A}_{RL} \cdot \Vect{W}_L + \Vect{A}_{RR} \cdot \Vect{W}_R \label{decoupled-systemsR}.
\end{eqnarray}

Without loss of generality, we assume $\epsilon_L \ll \epsilon_R$ and call the left subsystem \eqref{decoupled-systemsL} the stiff system, whereas the right subsystem \eqref{decoupled-systemsR} is non-stiff. After choosing a specific spatial discretization, i.e., the PVM method, a stability analysis can be performed.

\begin{remark}
  Note that the distinction between stiff and non-stiff region made by setting the collision rate in \eqref{e:collision_rate_adaptive} can also be much more arbitrary. We can have several, distinct regions with small collision rate $\epsilon_L$ or large collision rate $\epsilon_R$. A permutation of the variable vector $\Vect{W}$ can be performed to split the system to an upper and lower part with small or large collision rate, respectively. This will lead to more entries in the off-diagonal blocks $\Vect{A}_{RL}, \Vect{A}_{LR}$ and a larger bandwidth in the diagonal blocks $\Vect{A}_{LL}, \Vect{A}_{RR}$.
\end{remark}

\section{Spectral analysis}
TODO: examples for all equations, spatial discretizations, show different clusters

\section{Spatially adaptive time integration}
We now need to construct a time-stepping method with matching stability region. Therefore, we consider a special treatment of the stiff and non-stiff parts of the domain.

More precisely, we consider the transition from time step $n$ to time step $n+1$ and write the update as
\begin{equation}\label{decoupled-scheme}
        \left( \begin{array}{c}
        \Vect{W}_L^{n+1} \\
        \Vect{W}_R^{n+1} \\
      \end{array} \right) =
      \left( \begin{array}{cc}
        \widetilde{\Vect{A}}_{LL} & \widetilde{\Vect{A}}_{LR} \\
        \widetilde{\Vect{A}}_{RL} & \widetilde{\Vect{A}}_{RR} \\
      \end{array} \right)
       \left( \begin{array}{c}
        \Vect{W}_L^{n} \\
        \Vect{W}_R^{n} \\
      \end{array} \right),
\end{equation}
where we introduce the block-wise transition matrix $\widetilde{\Vect{A}} = \left( \begin{array}{cc}
        \widetilde{\Vect{A}}_{LL} & \widetilde{\Vect{A}}_{LR} \\
        \widetilde{\Vect{A}}_{RL} & \widetilde{\Vect{A}}_{RR} \\
      \end{array} \right)$.

The small relaxation time $\epsilon_L$ in the stiff part of the system leads to a severe time step constraint. In order to apply a tailored numerical integration scheme of the decoupled system, we apply a different time integration scheme in each domain. In the non-stiff domain, a standard forward Euler scheme with time step size $\Delta t$ is applied. In the stiff domain, a different scheme is necessary.

For comparison, we consider the following to standard schemes
\begin{itemize}
  \item[GFE:] Whole domain: Standard Forward Euler Method (global Forward Euler method)
  \item[GPFE:] Whole domain: Projective Forward Euler method (global Projective Forward Euler method)
\end{itemize}
and derive the following new schemes
\begin{itemize}
  \item[FE-FE:] Non-stiff domain: Forward Euler Method; Stiff domain: Forward Euler method
  \item[FE-PFE:] Non-stiff domain: Forward Euler Method; Stiff domain: Projective Forward Euler method
\end{itemize}
We call the methods FE-FE method and FE-PFE method, respectively.


\subsection{FE-FE scheme}
We first consider a standard forward Euler scheme with a smaller time step $\delta t$. For simplicity, we only consider the case $\Delta t = (K+1) \delta t$, for integer $K \in \mathbb{N}$.

The updates from the values $\Vect{W}^n$ to $\Vect{W}^{n+1}$ are performed in the following way
\begin{equation}\label{FE_update_R}
    \Vect{W}_R^{n+1} = \Vect{W}_R^{n} + \Delta t \left( \Vect{A}_{RL} \cdot \Vect{W}_L^{n} + \Vect{A}_{RR} \cdot \Vect{W}_R^{n} \right),
\end{equation}
for the non-stiff part of the domain and
\begin{eqnarray}\label{FE_update_L}
    \Vect{W}_L^{n,k+1} &=& \Vect{W}_L^{n,k} + \delta t \left( \Vect{A}_{LL} \cdot \Vect{W}_L^{n,k} + \Vect{A}_{LR} \cdot \Vect{W}_R^{n,k} \right), k = 0,\ldots,K\\
    \Vect{W}_L^{n+1} &=& \Vect{W}_L^{n,K+1},
\end{eqnarray}
for the stiff part of the domain with initialisations $\Vect{W}_L^{n,0} = \Vect{W}_L^{n}$, $\Vect{W}_R^{n,0} = \Vect{W}_R^{n}$. Note, that the intermediate values $\Vect{W}_R^{n,k}$ of the non-stiff part are computed via interpolation, i.e.,
\begin{eqnarray}\label{interpolation_R}
    \Vect{W}_R^{n,k+1} &=& \Vect{W}_R^{n} + (k+1) \cdot \delta t \cdot \frac{\Vect{W}_R^{n+1}-\Vect{W}_R^{n}}{\Delta t}, \\
                       &=& (k+1) \delta t \Vect{A}_{LR} \Vect{W}_L^{n} + (\Vect{I}+ \delta t (k+1) \Vect{A}_{RR} \Vect{W}_R^{n},
\end{eqnarray}

where the sparse form of the off-diagonal parts $\Vect{A}_{LR}$ and $\Vect{A}_{RL}$ allows for an efficient computation of the interpolation only at the interface.

\begin{theorem}\label{th_FE-FE}
    One time step of the FE-FE method with time step size $\Delta t$ in the non-stiff domain and time step size $\delta t$ in the stiff domain, for $\Delta t = (K+1) \delta t$ is given by the transition matrix $\widetilde{\Vect{A}}_{FE-FE}$ with block entries
    \begin{eqnarray*}
        \Vect{A}_{LL} &=& \left( \Vect{I} + \delta t \Vect{A}_{LL} \right)^{K+1} + \delta t^2 \sum_{k=0}^{K} (K-k) \left( \Vect{I} + \delta t \Vect{A}_{LL} \right)^{k} \Vect{A}_{LR} \Vect{A}_{RL}\\
        \Vect{A}_{LR} &=& \delta t \sum_{k=0}^{K} \left( \Vect{I} + \delta t \Vect{A}_{LL} \right)^{k} \Vect{A}_{LR} \left( \Vect{I} + (K-k)\delta t \Vect{A}_{RR} \right)\\
        \Vect{A}_{RL} &=& \Delta t \Vect{A}_{RL} \\
        \Vect{A}_{RR} &=& \Vect{I} + \Delta t \Vect{A}_{RR}.
    \end{eqnarray*}
\end{theorem}
\begin{proof}
  TODO write down proof from notes.
\end{proof}

As an example, we consider $K=1$, such that $\Delta t= 2\delta t$. Theorem \ref{th_FE-FE} then leads to the following transition matrix:
\begin{equation}
    \widetilde{\Vect{A}}_{FE-FE} = \left( \begin{array}{cc}
        \left( \Vect{I} + \delta t \Vect{A}_{LL} \right)^2 + \delta t^2 \Vect{A}_{LR} \Vect{A}_{RL}& 2 \delta t \Vect{A}_{LR} + \delta t^2 \left(\Vect{A}_{LR} \Vect{A}_{RR} + \Vect{A}_{LL} \Vect{A}_{LR}\right)\\
        \Delta t \Vect{A}_{RL} & \Vect{I} + \Delta t \Vect{A}_{RR}
      \end{array} \right),
\end{equation}
which can be written as
\begin{equation}
    \widetilde{\Vect{A}}_{FE-FE} = \Vect{I} + \Delta t \left( \begin{array}{cc}
        \Vect{A}_{LL} & \Vect{A}_{LR} \\
        \Vect{A}_{RL} & \Vect{A}_{RR} \\
      \end{array} \right) + \delta t^2 \left( \begin{array}{cc}
        \Vect{A}_{LL}^2 + \Vect{A}_{LR} \Vect{A}_{RL} & \Vect{A}_{LL} \Vect{A}_{LR} + \Vect{A}_{LR} \Vect{A}_{RL}\\
        \Vect{0} & \Vect{0} \\
      \end{array} \right)
\end{equation}


TODO: write down proof that consistency error is $\mathcal{O}(\Delta t)$

\subsection{FE-PFE scheme}
We keep a standard forward Euler scheme in the non-stiff region but employ a Projective Forward Euler scheme with $K$ inner Forward Euler steps of smaller time step $\delta t << \Delta t$ in the stiff domain.

The update and interpolation of the non-stiff values from Equations \eqref{FE_update_R} and \eqref{interpolation_R} are the same. The Projective Forward Euler scheme uses $K$ inner Forward Euler steps and subsequent extrapolation over the remaining time interval
\begin{eqnarray}
    \Vect{W}_L^{n,k+1} &=& \Vect{W}_L^{n,k} + \delta t \left( \Vect{A}_{LL} \cdot \Vect{W}_L^{n,k} + \Vect{A}_{LR} \cdot \Vect{W}_R^{n,k} \right), k = 0,\ldots,K\\
    \Vect{W}_L^{n+1} &=& \Vect{W}_L^{n,K+1} + \left(\Delta t - (K+1) \delta t\right) \frac{\Vect{W}_L^{n,K+1} - \Vect{W}_L^{n,K}}{\delta t},
\end{eqnarray}

\begin{theorem}\label{th_FE-PFE}
    One time step of the FE-PFE method with time step size $\Delta t$ in the non-stiff domain and $K$ time steps of size $\delta t$ with subsequent extrapolation in the stiff domain is given by the transition matrix $\widetilde{\Vect{A}}_{FE-PFE}$ with block entries
    \begin{eqnarray*}
        \Vect{A}_{LL} &=& \left( \Vect{I} + (\Delta t - K \delta t) \Vect{A}_{LL} \right) \left( \delta t^2 \sum_{k=0}^{K-1} (K-1-k) \left( \Vect{I} + \delta t \Vect{A}_{LL} \right)^k \Vect{A}_{LR} \Vect{A}_{RL} + \left( \Vect{I} + \delta t \Vect{A}_{LL} \right)^K \right) \\
        \Vect{A}_{LR} &=& \left( \Vect{I} + (\Delta t - K \delta t) \Vect{A}_{LL} \right) \delta t \sum_{k=0}^{K-1} \left( \Vect{I} + \delta t \Vect{A}_{LL} \right)^k \Vect{A}_{LR} \left( \Vect{I} + (K-1-k)\delta t \Vect{A}_{RR} \right) \\
                      & & + (\Delta t -K \delta t) \Vect{A}_{LR} \left( \Vect{I} + K \delta t \Vect{A}_{RR} \right) \\
        \Vect{A}_{RL} &=& \Delta t \Vect{A}_{RL} \\
        \Vect{A}_{RR} &=& \Vect{I} + \Delta t \Vect{A}_{RR}.
    \end{eqnarray*}
\end{theorem}
\begin{proof}
  TODO write down proof from notes.
\end{proof}

As an example, we consider $K=1$, which is often used for PFE schemes. Theorem \ref{th_FE-PFE} then leads to the following transition matrix:
\begin{equation}
    \widetilde{\Vect{A}}_{FE-PFE} = \left( \begin{array}{cc}
        \left( \Vect{I} + (\Delta t - \delta t) \Vect{A}_{LL} \right) \left( \Vect{I} + \delta t \Vect{A}_{LL} \right) + \delta t (\Delta t - \delta t) \Vect{A}_{LR} \Vect{A}_{RL} & (\Delta t - \delta t) \left( \Vect{A}_{LR} + \delta t \Vect{A}_{LR} \Vect{A}_{RR} \right) \\
        \Delta t \Vect{A}_{RL} & \Vect{I} + \Delta t \Vect{A}_{RR}
      \end{array} \right),
\end{equation}
which can be written as
\begin{equation}
    \widetilde{\Vect{A}}_{FE-PFE} = \Vect{I} + \Delta t \left( \begin{array}{cc}
        \Vect{A}_{LL} & \Vect{A}_{LR} \\
        \Vect{A}_{RL} & \Vect{A}_{RR} \\
      \end{array} \right) + \left( \begin{array}{cc}
        \delta t (\Delta t - \delta t)  \left( \Vect{A}_{LL}^2 + \Vect{A}_{LR} \Vect{A}_{RL} \right) & -\delta t \Vect{A}_{LR} + \delta t (\Delta t - \delta t) \Vect{A}_{LR} \Vect{A}_{RR}\\
        \Vect{0} & \Vect{0} \\
      \end{array} \right)
\end{equation}

TODO: write down proof that consistency error is $\mathcal{O}(\Delta t)$

\begin{remark}
    TODO: possible generalization for RK methods
\end{remark}

\section{Stability analysis}

TODO


%\subsection{Semi-discrete system}
%Example: Lax-Friedrich

%TODO: use $\Vect{Q} = \frac{\Delta x}{\Delta t} \Vect{I}$. Do LSA. Can eigenvalues be estimated using Gershgorin circles?

%\subsection{FE-FE scheme}
%\subsection{FE-PFE scheme}


